Sublinear Algorithms and Lower Bounds for Estimating MST and TSP Cost in General Metrics

We consider the design of sublinear space and query complexity algorithms for estimating the cost of a minimum spanning tree (MST) and the cost of a minimum traveling salesman (TSP) tour in a metric on $n$ points. We first consider the $o(n)$-space regime and show that, when the input is a stream of all $\binom{n}{2}$ entries of the metric, for any $\alpha \ge 2$, both MST and TSP cost can be $\alpha$-approximated using $\tilde{O}(n/\alpha)$ space, and that $\Omega(n/\alpha^2)$ space is necessary for this task. Moreover, we show that even if the streaming algorithm is allowed $p$ passes over a metric stream, it still requires $\tilde{\Omega}(\sqrt{n/\alpha p^2})$ space. We next consider the semi-streaming regime, where computing even the exact MST cost is easy and the main challenge is to estimate TSP cost to within a factor that is strictly better than $2$. We show that, if the input is a stream of all edges of the weighted graph that induces the underlying metric, for any $\varepsilon > 0$, any one-pass $(2-\varepsilon)$-approximation of TSP cost requires $\Omega(\varepsilon^2 n^2)$ space; on the other hand, there is an $\tilde{O}(n)$ space two-pass algorithm that approximates the TSP cost to within a factor of 1.96. Finally, we consider the query complexity of estimating metric TSP cost to within a factor that is strictly better than $2$, when the algorithm is given access to a matrix that specifies pairwise distances between all points. For MST estimation in this model, it is known that a $(1+\varepsilon)$-approximation is achievable with $\tilde{O}(n/\varepsilon^{O(1)})$ queries. We design an algorithm that performs $\tilde{O}(n^{1.5})$ distance queries and achieves a strictly better than $2$-approximation when either the metric is known to contain a spanning tree supported on weight-$1$ edges or the algorithm is given access to a minimum spanning tree of the graph.

==> REF.tex <==
@string{STOC = "Proceedings of the Symposium on Theory of Computing"}

@string{FOCS = "Proceedings of the Symposium on Foundations of Computer Science"}

@string{SODA = "Proceedings of the ACM-SIAM Symposium on Discrete Algorithms"}

@article{behnezhad2021time,
	title={Time-Optimal Sublinear Algorithms for Matching and Vertex Cover},
	author={Behnezhad, Soheil},
	journal={arXiv preprint arXiv:2106.02942},
	year={2021}
}


@article{vizing1964estimate,
	title={On an estimate of the chromatic class of a p-graph},
	author={Vizing, Vadim G},
	journal={Discret Analiz},
	volume={3},
	pages={25--30},
	year={1964}
}

@article{DolevF92,
  author    = {Danny Dolev and
               Tom{\'{a}}s Feder},
  title     = {Determinism vs. Nondeterminism in Multiparty Communication Complexity},
  journal   = {{SIAM} J. Comput.},
  volume    = {21},
  number    = {5},
  pages     = {889--895},
  year      = {1992},
}

@article{kremer1999randomized,
	title={On randomized one-round communication complexity},
	author={Kremer, Ilan and Nisan, Noam and Ron, Dana},
	journal={Computational Complexity},
	volume={8},
	number={1},
	pages={21--49},
	year={1999},
	publisher={Springer}
}


@article{prahladhlecture,
	title={Lecture notes on communication complexity},
	author={Prahladh Harsha},
	year={2011},
	url={https://www.tifr.res.in/~prahladh/teaching/2011-12/comm/lectures/l12.pdf}
}

@techreport{christofides1976worst,
  title={Worst-case analysis of a new heuristic for the travelling salesman problem},
  author={Christofides, Nicos},
  year={1976},
  institution={Carnegie-Mellon Univ Pittsburgh Pa Management Sciences Research Group}
}


@article{abs-1305-4696,
  author    = {Mark Braverman and
               Faith Ellen and
               Rotem Oshman and
               Toniann Pitassi and
               Vinod Vaikuntanathan},
  title     = {Tight Bounds for Set Disjointness in the Message Passing Model},
  journal   = {CoRR},
  volume    = {abs/1305.4696},
  year      = {2013},
  url       = {http://arxiv.org/abs/1305.4696},
}

@article{Lin91,
  author    = {Jianhua Lin},
  title     = {Divergence measures based on the Shannon entropy},
  journal   = {{IEEE} Trans. Inf. Theory},
  volume    = {37},
  number    = {1},
  pages     = {145--151},
  year      = {1991},
}

@article{Bar-YossefJKS04,
  author    = {Ziv Bar{-}Yossef and
               T. S. Jayram and
               Ravi Kumar and
               D. Sivakumar},
  title     = {An information statistics approach to data stream and communication
               complexity},
  journal   = {J. Comput. Syst. Sci.},
  volume    = {68},
  number    = {4},
  pages     = {702--732},
  year      = {2004},
}

@article{BravermanR14,
  author    = {Mark Braverman and
               Anup Rao},
  title     = {Information Equals Amortized Communication},
  journal   = {{IEEE} Trans. Inf. Theory},
  volume    = {60},
  number    = {10},
  pages     = {6058--6069},
  year      = {2014},
}

@inproceedings{JowhariST2011,
    title={Tight bounds for Lp samplers, finding duplicates in streams, and related problems},
    author={Jowhari, Hossein and Sa{\u{g}}lam, Mert and Tardos, G{\'a}bor},
    booktitle={Proceedings of the thirtieth ACM SIGMOD-SIGACT-SIGART symposium on Principles of database systems},
    pages={49--58},
    year={2011},
    organization={ACM}
}

@inproceedings{kapralov2020space,
  title={Space efficient approximation to maximum matching size from uniform edge samples},
  author={Kapralov, Michael and Mitrovi{\'c}, Slobodan and Norouzi-Fard, Ashkan and Tardos, Jakab},
  booktitle={Proceedings of the Fourteenth Annual ACM-SIAM Symposium on Discrete Algorithms},
  pages={1753--1772},
  year={2020},
  organization={SIAM}
}

@article{chen2020sublinear,
  title={Sublinear Algorithms and Lower Bounds for Metric TSP Cost Estimation},
  author={Chen, Yu and Kannan, Sampath and Khanna, Sanjeev},
  journal={arXiv preprint arXiv:2006.05490},
  year={2020}
}

@inproceedings{momke2011approximating,
  title={Approximating graphic TSP by matchings},
  author={M{\"o}mke, Tobias and Svensson, Ola},
  booktitle={2011 IEEE 52nd Annual Symposium on Foundations of Computer Science},
  pages={560--569},
  year={2011},
  organization={IEEE}
}

@article{czumaj2009estimating,
  title={Estimating the weight of metric minimum spanning trees in sublinear time},
  author={Czumaj, Artur and Sohler, Christian},
  journal={SIAM Journal on Computing},
  volume={39},
  number={3},
  pages={904--922},
  year={2009},
  publisher={SIAM}
}

@inproceedings{focs/MomkeS11,
	author    = {Tobias M{\"{o}}mke and
	Ola Svensson},
	title     = {Approximating Graphic {TSP} by Matchings},
	booktitle = {{IEEE} 52nd Annual Symposium on Foundations of Computer Science, {FOCS}
	2011, Palm Springs, CA, USA, October 22-25, 2011},
	pages     = {560--569},
	year      = {2011},
	url       = {https://doi.org/10.1109/FOCS.2011.56},
	doi       = {10.1109/FOCS.2011.56},
}

@article{GoldreichR02,
	author    = {Oded Goldreich and
	Dana Ron},
	title     = {Property Testing in Bounded Degree Graphs},
	journal   = {Algorithmica},
	volume    = {32},
	number    = {2},
	pages     = {302--343},
	year      = {2002}
}

@article{PR07,
	author    = {Michal Parnas and
	Dana Ron},
	title     = {Approximating the minimum vertex cover in sublinear time and a connection
	to distributed algorithms},
	journal   = {Theor. Comput. Sci.},
	volume    = {381},
	number    = {1-3},
	pages     = {183--196},
	year      = {2007}
}

@article{CQ18,
	author    = {Chandra Chekuri and
	Kent Quanrud},
	title     = {Fast Approximations for Metric-{TSP} via Linear Programming},
	journal   = {CoRR},
	volume    = {abs/1802.01242},
	year      = {2018}
}

@inproceedings{CQ17,
	author    = {Chandra Chekuri and
	Kent Quanrud},
	title     = {Approximating the Held-Karp Bound for Metric {TSP} in Nearly-Linear
	Time},
	booktitle = {58th {IEEE} Annual Symposium on Foundations of Computer Science, {FOCS}
	2017, Berkeley, CA, USA, October 15-17, 2017},
	pages     = {789--800},
	year      = {2017}
}

@inproceedings{NguyenO08,
	author    = {Huy N. Nguyen and
	Krzysztof Onak},
	title     = {Constant-Time Approximation Algorithms via Local Improvements},
	booktitle = {49th Annual {IEEE} Symposium on Foundations of Computer Science, {FOCS}
	2008, October 25-28, 2008, Philadelphia, PA, {USA}},
	pages     = {327--336},
	year      = {2008},
	biburl    = {https://dblp.org/rec/bib/conf/focs/NguyenO08},
}

@misc{onakpersonalcommunication,
	author = {Onak, Krzysztof and Ron, Dana and Rosen, Michal and Rubinfeld, Ronitt},
	date = "July 2019",
	howpublished = "Personal communication",
	year={2019}
}

@inproceedings{kapralov2020space,
	title={Space efficient approximation to maximum matching size from uniform edge samples},
	author={Kapralov, Michael and Mitrovi{\'c}, Slobodan and Norouzi-Fard, Ashkan and Tardos, Jakab},
	booktitle={Proceedings of the Fourteenth Annual ACM-SIAM Symposium on Discrete Algorithms},
	pages={1753--1772},
	year={2020},
	organization={SIAM}
}

@inproceedings{adamaszek2018new,
	title={New approximation algorithms for (1, 2)-tsp},
	author={Adamaszek, Anna and Mnich, Matthias and Paluch, Katarzyna},
	booktitle={45th International Colloquium on Automata, Languages, and Programming (ICALP 2018)},
	year={2018},
	organization={Schloss Dagstuhl-Leibniz-Zentrum fuer Informatik}
}

@inproceedings{Vygen2012_Survey,
	title={New approximation algorithms for the TSP},
	author={Jens Vygen},
	year={2012}
}

@article{KarpinskiLS15,
	author    = {Marek Karpinski and
	Michael Lampis and
	Richard Schmied},
	title     = {New inapproximability bounds for {TSP}},
	journal   = {J. Comput. Syst. Sci.},
	volume    = {81},
	number    = {8},
	pages     = {1665--1677},
	year      = {2015}
}

@inproceedings{SeboZ16,
	author    = {Andr{\'{a}}s Seb{\"{o}} and
	Anke van Zuylen},
	title     = {The Salesman's Improved Paths: {A} 3/2+1/34 Approximation},
	booktitle = {{IEEE} 57th Annual Symposium on Foundations of Computer Science, {FOCS}
	2016, 9-11 October 2016, Hyatt Regency, New Brunswick, New Jersey,
	{USA}},
	pages     = {118--127},
	year      = {2016}
}

@article{Gao18,
	author    = {Zhihan Gao},
	title     = {On the Metric s-t Path Traveling Salesman Problem},
	journal   = {{SIAM} Review},
	volume    = {60},
	number    = {2},
	pages     = {409--426},
	year      = {2018}
}

@inproceedings{TraubV18,
	author    = {Vera Traub and
	Jens Vygen},
	title     = {Beating the Integrality Ratio for s-t-Tours in Graphs},
	booktitle = {59th {IEEE} Annual Symposium on Foundations of Computer Science, {FOCS}
	2018, Paris, France, October 7-9, 2018},
	pages     = {766--777},
	year      = {2018}
}

@article{MnichM18,
	author    = {Matthias Mnich and
	Tobias M{\"{o}}mke},
	title     = {Improved integrality gap upper bounds for traveling salesperson problems
	with distances one and two},
	journal   = {European Journal of Operational Research},
	volume    = {266},
	number    = {2},
	pages     = {436--457},
	year      = {2018}
}

@article{TraubV19,
	author    = {Vera Traub and
	Jens Vygen},
	title     = {Approaching 3/2 for the \emph{s}-\emph{t}-path {TSP}},
	journal   = {J. {ACM}},
	volume    = {66},
	number    = {2},
	pages     = {14:1--14:17},
	year      = {2019},
	url       = {https://doi.org/10.1145/3309715},
	doi       = {10.1145/3309715},
	timestamp = {Thu, 09 May 2019 13:10:56 +0200},
	biburl    = {https://dblp.org/rec/bib/journals/jacm/TraubV19},
	bibsource = {dblp computer science bibliography, https://dblp.org}
}


@article{ChazelleRT05,
	author    = {Bernard Chazelle and
	Ronitt Rubinfeld and
	Luca Trevisan},
	title     = {Approximating the Minimum Spanning Tree Weight in Sublinear Time},
	journal   = {{SIAM} J. Comput.},
	volume    = {34},
	number    = {6},
	pages     = {1370--1379},
	year      = {2005}
}


@article{AnKS15,
	author    = {Hyung{-}Chan An and
	Robert D. Kleinberg and
	David B. Shmoys},
	title     = {Improving Christofides' Algorithm for the s-t Path {TSP}},
	journal   = {J. {ACM}},
	volume    = {62},
	number    = {5},
	pages     = {34:1--34:28},
	year      = {2015}
}

@inproceedings{berman20068,
	title={8/7-approximation algorithm for (1, 2)-TSP},
	author={Berman, Piotr and Karpinski, Marek},
	booktitle={Proceedings of the seventeenth annual ACM-SIAM symposium on Discrete algorithm},
	pages={641--648},
	year={2006},
	organization={Society for Industrial and Applied Mathematics}
}

@article{mucha2014frac,
	title={$\frac{13}{9}$-Approximation for Graphic TSP},
	author={Mucha, Marcin},
	journal={Theory of computing systems},
	volume={55},
	number={4},
	pages={640--657},
	year={2014},
	publisher={Springer}
}

@article{karpinski2015new,
	title={New inapproximability bounds for TSP},
	author={Karpinski, Marek and Lampis, Michael and Schmied, Richard},
	journal={Journal of Computer and System Sciences},
	volume={81},
	number={8},
	pages={1665--1677},
	year={2015},
	publisher={Elsevier}
}

@techreport{christofides1976worst,
	title={Worst-case analysis of a new heuristic for the travelling salesman problem},
	author={Christofides, Nicos},
	year={1976},
	institution={Carnegie-Mellon Univ Pittsburgh Pa Management Sciences Research Group}
}

@inproceedings{assadi2017estimating,
	title={On estimating maximum matching size in graph streams},
	author={Assadi, Sepehr and Khanna, Sanjeev and Li, Yang},
	booktitle={Proceedings of the Twenty-Eighth Annual ACM-SIAM Symposium on Discrete Algorithms},
	pages={1723--1742},
	year={2017},
	organization={SIAM}
}

@misc{sublinear71,
	howpublished = "\url{https://sublinear.info/71}"
}

@article{czumaj2009estimating,
	title={Estimating the weight of metric minimum spanning trees in sublinear time},
	author={Czumaj, Artur and Sohler, Christian},
	journal={SIAM Journal on Computing},
	volume={39},
	number={3},
	pages={904--922},
	year={2009},
	publisher={SIAM}
}

@article{goncharov1944some,
	title={Some facts from combinatorics},
	author={Goncharov, VL},
	journal={Izvestia Akad. Nauk. SSSR, Ser. Mat},
	volume={8},
	pages={3--48},
	year={1944}
}

@article{kremer1999randomized,
	title={On randomized one-round communication complexity},
	author={Kremer, Ilan and Nisan, Noam and Ron, Dana},
	journal={Computational Complexity},
	volume={8},
	number={1},
	pages={21--49},
	year={1999},
	publisher={Springer}
}

@article{dirac1952some,
	title={Some theorems on abstract graphs},
	author={Dirac, Gabriel Andrew},
	journal={Proceedings of the London Mathematical Society},
	volume={3},
	number={1},
	pages={69--81},
	year={1952},
	publisher={Wiley Online Library}
}

@inproceedings{Yao87,
	author    = {Andrew Chi{-}Chih Yao},
	title     = {Lower Bounds to Randomized Algorithms for Graph Properties (Extended
	Abstract)},
	booktitle = {28th Annual Symposium on Foundations of Computer Science, Los Angeles,
	California, USA, 27-29 October 1987},
	pages     = {393--400},
	year      = {1987}
}

@article{yoshida2012improved,
	title={Improved constant-time approximation algorithms for maximum matchings and other optimization problems},
	author={Yoshida, Yuichi and Yamamoto, Masaki and Ito, Hiro},
	journal={SIAM Journal on Computing},
	volume={41},
	number={4},
	pages={1074--1093},
	year={2012},
	publisher={SIAM}
}

@article{haastad2001some,
	title={Some optimal inapproximability results},
	author={H{\aa}stad, Johan},
	journal={Journal of the ACM (JACM)},
	volume={48},
	number={4},
	pages={798--859},
	year={2001},
	publisher={ACM}
}

@inproceedings{bogdanov2002lower,
	title={A lower bound for testing 3-colorability in bounded-degree graphs},
	author={Bogdanov, Andrej and Obata, Kenji and Trevisan, Luca},
	booktitle={The 43rd Annual IEEE Symposium on Foundations of Computer Science, 2002. Proceedings.},
	pages={93--102},
	year={2002},
	organization={IEEE}
}

@article{papadimitriou1993traveling,
	title={The traveling salesman problem with distances one and two},
	author={Papadimitriou, Christos H and Yannakakis, Mihalis},
	journal={Mathematics of Operations Research},
	volume={18},
	number={1},
	pages={1--11},
	year={1993},
	publisher={INFORMS}
}

@inproceedings{assadi2019sublinear,
	title={Sublinear algorithms for ({\(\Delta\)}+ 1) vertex coloring},
	author={Assadi, Sepehr and Chen, Yu and Khanna, Sanjeev},
	booktitle={Proceedings of the Thirtieth Annual ACM-SIAM Symposium on Discrete Algorithms},
	pages={767--786},
	year={2019},
	organization={Society for Industrial and Applied Mathematics}
}

@inproceedings{onak2012near,
	title={A near-optimal sublinear-time algorithm for approximating the minimum vertex cover size},
	author={Onak, Krzysztof and Ron, Dana and Rosen, Michal and Rubinfeld, Ronitt},
	booktitle={Proceedings of the twenty-third annual ACM-SIAM symposium on Discrete Algorithms},
	pages={1123--1131},
	year={2012},
	organization={Society for Industrial and Applied Mathematics}
}

@article{momke2016removing,
	title={Removing and adding edges for the traveling salesman problem},
	author={M{\"o}mke, Tobias and Svensson, Ola},
	journal={Journal of the ACM (JACM)},
	volume={63},
	number={1},
	pages={2},
	year={2016},
	publisher={ACM}
}

@article{sebo2014shorter,
	title={Shorter tours by nicer ears: 7/5-Approximation for the graph-TSP, 3/2 for the path version, and 4/3 for two-edge-connected subgraphs.},
	author={Seb{\"o}, Andr{\'a}s and Vygen, Jens},
	journal={Combinatorica},
	volume={34},
	number={5},
	pages={597--629},
	year={2014}
}

@book{west1996introduction,
	title={Introduction to graph theory},
	author={West, Douglas B.},
	year={1996},
	publisher={Prentice-Hall Inc.}
}

@inproceedings{karlin2021slightly,
	title={A (slightly) improved approximation algorithm for metric TSP},
	author={Karlin, Anna R and Klein, Nathan and Gharan, Shayan Oveis},
	booktitle={Proceedings of the 53rd Annual ACM SIGACT Symposium on Theory of Computing},
	pages={32--45},
	year={2021}
}


==> overview.tex <==
\section{Technical Overview}

\subsection{Algorithmic Techniques}

%\newcommand{\cov}{{\mathsf{cov}}}
%\newcommand{\adv}{\mathsf{adv}}

Our streaming algorithm for MST estimation (\Cref{thm: 1 pass alpha MST upper}) utilizes a rather natural idea. We sample $O(n/\alpha)$ vertices and maintain a MST $T'$ over them. For remaining vertices, we maintain an estimate of the cost of connecting them to the nearest vertex in $T'$. We show that these estimates can be suitable combined to oibtain an $\alpha$-approximation of MST cost.
%utilizes a standard randomized approach based on sampling a random subset of vertices and record the distances from other vertices to them. 
In this subsection we focus on providing a high-level overview of the algorithms for TSP estimation.

It is well-known that $\mst\le \tsp\le 2\cdot \mst$ holds for any graph/metric, since we can construct a TSP-tour by doubling all edges of a MST (and then shortcut the obtained walk into a tour).
Since the MST weight of a graph/metric can be exactly computed by a one-pass $\tilde O(n)$ space algorithm (the greedy algorithm) in the streaming model, and can be approximated to within a factor of $(1+\eps)$ by performing $\tilde O(n)$ queries in the query model \cite{czumaj2009estimating}, to obtain a factor $(2-\eps)$ approximation for $\tsp$, it suffices to establish either $\tsp\ge (1+\eps)\cdot\mst$ or $\tsp\le (2-\eps)\cdot\mst$ holds.
From the approach due to \cite{christofides1976worst}, the minimum weight of a perfect matching on the set of all odd-degree vertices in a MST can immediately gives us the answer. However, obtaining a good approximation to the minimum weight of such a perfect matching appears hard to do, both for semi-streaming algorithms and for a query algorithm that performs $o(n^2)$ queries, even if we are given a MST at the start. To get around this issue, we consider an alternative measure, called the \emph{cover advantage}, that turns out to be more tractable in both models.


\paragraph{Cover Advantage.} Let $T$ be a MST of the input graph/metric. For an edge $f\in E(T)$ and an edge $e\notin E(T)$, we say that $f$ is \emph{covered} by $e$, iff $f$ belongs to the unique tree-path in $T$ connecting the endpoints of $e$. 
For a set $E'$ of edges, we denote by $\cov(E', T)$ the set of all edges in $E(T)$ that are covered by at least one edge in $E'$. The \emph{cover advantage} of $E'$, denoted by $\adv(E')$, is defined to be the difference between the total weight of all edges in $\cov(E', T)$ and the total weight of all edges in $E'$. 
Intuitively, if a single-edge set $\set{e}$ where $e=(u,v)$ has cover advantage $c$, then we can construct a tour by starting from some Euler-tour of $T$ and replacing the segment corresponding to the tree path of $T$ connecting $u$ to $v$ by the single edge $e$, and thereby ``saving a cost of $c$'' from $2\cdot \mst$, the cost of the Euler-tour obtained by doubling MST edges.
Generalizing this idea, we show that if there exists a set $E'$ with cover advantage bounded away from $0$ (at least $\eps\cdot \mst$), then $\tsp\le (2-\eps/2)\cdot \mst$. Conversely, if there does not exist any set $E'$ with aover advantage bounded away from $\mst/2$ (at most $(1/2-\eps/2)\cdot \mst$), then $\tsp\ge (1+\eps)\cdot \mst$.
%if the maximum cover advantage of any subset $E'$ of edges is bounded away from $0$ (at least $\eps\cdot \mst$), then $\tsp\le (2-\eps/2)\cdot \mst$, and if it is bounded away from $\mst/2$ (at most $(1/2-\eps/2)\cdot \mst$), then $\tsp\ge (1+\eps)\cdot \mst$.
In fact, we show that the same hold for a more restricted notion called \emph{special cover advantage}, which is defined to be the maximum cover advantage of any subset $E'$ of edges that have at least one endpoints being a special vertex in $T$ (a vertex $v$ is called a \emph{special vertex} of $T$ iff $\deg_T(v)\ne 2$).
Therefore, to obtain a better-than-factor-2 approximation for $\tsp$, it suffices to obtain a constant-factor approximation for the maximum cover advantage or the maximum special cover advantage.

\paragraph{Estimating maximum cover advantage in the streaming setting.}
We construct a one-pass streaming algorithm $O(1)$-estimating the maximum cover advantage, which leads to a two-pass algorithm in \Cref{thm: 2 pass TSP upper} where in the first pass we only compute a MST of the input graph. We store edges with substantial cover advantage with respect to the MST in a greedy manner. Since all edges appear in the stream, it can be shown that, if we end up not discovering a large cover advantage, then the real maximum cover advantage is indeed small (bounded away from $\mst/2$).

\paragraph{Estimating maximum cover advantage in the query model.} The task of obtaining a constant-factor approximation to maximum cover advantage is distinctly more challenging in the query model, even if we are gievn access to a MST.
This is our main algorithmic constribution.
We design an $\tilde O(n^{1.5})$-query algorithm for estimating the maximum cover advantage when either a MST is explicitly given or we can assume that the MST is supported on weight-$1$ edges. Note that the latter case generalizes graphic TSP studied in \cite{chen2020sublinear}.
%
%In particular, we are not even given a MST in the first place. 
Although the weight of a MST can be accurately approximated with $\tilde O(n)$ queries, computing a MST (or even a spanning tree with cost at most $(2-\eps)\cdot\mst$) requires $\Omega(n^2)$ queries, as shown in \cite{chen2020sublinear}.
Therefore, to be able to exploit the power of the cover advantage technique, we need some additional MST-related properties of the input metric. Specifically, we need addtional information of the MST in the following two aspects:
\begin{enumerate}
\item What structure does the MST have?
\item What are the weights of the MST edges?
\end{enumerate}

%We design an $\tilde O(n^{1.5})$-query algorithm for estimating the maximum cover advantage when either a MST is explicitly given or we can assume that the MST is supported on weight-$1$ edges. Note that the latter case generalizes graphic TSP studied in \cite{chen2020sublinear}.
%Even if we are gievn access to a MST, this is our main algorithmic constribution.

The two special cases we explored in this paper reflect the two aspects mentioned above. In the first special case, we assume that the MST consists of only weight-$1$ edges, but make no assumptions on its structure.
In the second special case, we assume that we are given the structure of the MST, but make no assumptions on its edge weights.

In fact, the algorithms for two special cases are more or less similar. To illustrate the ideas behind them, it might be instructive to consider the following two examples. In the first example, we are given a MST $T$ on $V$ that has at most $O(\sqrt{n})$ leaves. 
We can simply query the distances between all pairs $u,v\in V$ where $u$ is a special vertex of $T$, and then use the obtained information to compute the maximum special cover advantage, which takes $\tilde O(n^{1.5})$ queries since there can be at most $O(\sqrt n)$ special vertices (or in fact we can even query the distances between all pairs of odd-degree vertices in $T$ and compute the minimum weight perfect matching on them).
In the second example, we given a MST $T$ on $V$ which is a star graph centered at a vertex $r\in V$, and all edges have weight $1$. Note that, since all edge weights are integers, in this case the distances between every pair of vertices in $V\setminus \set{r}$ is either $1$ or $2$, and it is not hard to see that the maximum cover advantage is exactly the size of a maximum weight-$1$ matching on $V\setminus \set{r}$.
Therefore, we can adapt the algorithm from \cite{behnezhad2021time} to obtain an $O(1)$-approximation of the maximum weight-$1$ matching size, using $\tilde{O}(n)$ queries.
Note that, in this case we obtain an estimate of the maximum cover advantage without computing a set of edges that achieves it.

Taking a step back, we observe that, in the first example where the number of special vertices is small, the cover advantage can be computed in a local and exhaustive manner, while in the second example where the number of special vertices is large, the cover advantage has to be estimated in a global and ``superficial'' manner. Intuitively, our query algorithms interpolate between these two approaches in an organic manner.

We now provide more details of our query algorithms in the two special cases. We first consider the special case where we are given the structure of a MST.

\paragraph{When MST is given:} We root the given MST $T$ at an arbitrary vertex. For each vertex $v\in V$, we say that it is \emph{light} iff the subtree of $T$ rooted at $v$, denoted by $T_v$, contains at most $\sqrt n$ vertices, and we call $T_v$ a \emph{light subtree} of $T$. On the one hand, the cover advantage that are local at some light subtree (achieved by edges with both endpoints in the same light subtree) can be efficiently estimated in an exhaustive manner. On the other hand, if we peel off all light subtrees from $T$, then the remaining subtree, that we denote by $T'$, contains at most $\sqrt{n}$ leaves, and therefore the special cover advantage achieved by any set of edges with at least one endpoint being a special vertex of $T'$ can also be computed in an exhaustive manner. The only type of cover advantage that is not yet computed are the one achieved by edges with endpoints in different light subtrees. We then observe that the light subtrees hanged at $T$ are similar to the edges of a star graph hanged at its root, and eventually manage to adapt the algorithm from \cite{behnezhad2021time} in a delicate way to estimate the cover advantage by edges of this type.

\paragraph{When MST consists of only weight-$1$ edges:} %We now consider the special case where the MST consists of only weight-$1$ edges. 
This special case appears trickier since we do not know the structure of a MST at the start, and there may not even be a unique MST.
To circumvent this, we need to utilize the following technical result of \cite{chen2020sublinear}:
Let $G_1$ be the graph on $V$ induced by all weight-$1$ edges in the given metric, then if $G_1$ contains a size-$s$ matching consisting of only edges in $2$-edge-connected components of $G_1$, then $\tsp\le 2n-\Omega(s)$.
This result allows us to construct a local procedure that explores some neighborhood of the unknown graph $G_1$ up to a certain size, such that in the end we either reconstruct a size-$\sqrt n$ subgraph of the (locally) unique MST, or certify that a set of $\Omega(\sqrt n)$ vertices belong to some $2$-edge-connected components of $G_1$,
which will be later collected to estimate the maximum weight-$1$ matching size on.

We then use this local procedure on a set of vertices randomly sampled from $V$. Let $T$ be a MST. Intuitively, if the total size of light subtrees of $T$ is non-negligible, then with high probability some of the sampled vertices will lie in light subtrees of $T$, and we can obtain an estimate of the local cover advantage within subtrees. If the total size of light subtrees is negligible, then $T'$ has roughly the same size as $T$, which means that $T$ is close to the first instructive example mentioned before -- a tree with only $O(\sqrt{n})$ special vertices. Then we can apply the local procedure to $\Omega(\sqrt{n})$ sampled vertices, to almost reconstruct the whole tree $T$, and the rest of the algorithm is similar to the algorithm in the first special case.










\subsection{Lower Bound Techniques}

%As it turns out, proving a space lower bound for streaming algorithms in metric streams is essentially different from (and also harder than) the same task in graph streams.

As our algorithmic results illustrate that metric streams are more powerful than graph stream, it is perhaps not surprising that proving space lower bounds for metrics streams turns out to me a more challenging task that requires new tools.
To illustrate this point, it might be instructive to consider the following simplified versions of metric and graph streams. Let $G$ be a graph.
%
\begin{itemize}
\item Unweighted Graph Stream: a sequence that contains all edges of $E(G)$, and the same edge may appear more than once in the stream;
\item Unweighted Metric Stream: a sequence that contains, for each pair $u,v$ of $V(G)$, a symbol $f(u,v)$ indicating whether or not the edge $(u,v)$ belongs to $E(G)$.
%, and the same tuple $(u,v,f(u,v))$ may appear more than once in the stream.
\end{itemize}
%
Note that in unweighted metric streams, the non-edge information between pairs of vertices are also explicitly given (as the edge information), as opposed to being given implicitly in the unweighted graph stream. This seemingly unimportant distinction, unexpectedly, makes proving lower bounds for several problems much harder in unweighted metric streams than in unweighted graph streams. 

For example, consider the problem of deciding whether the input graph is a clique.
On the one hand, to prove a space lower bound for streaming algorithms in unweighted graph streams, we consider the following two-player one-way communication game: Alice is given a graph $G_A$ and Bob is given a graph $G_B$ on a common vertex set $V$, and Alice and Bob want to decide if $G_A\cup G_B$ is the complete graph on $V$. It is easy to show that this communication game has back-and-forth communication complexity $\Omega(n^2)$. In fact, Alice's input graph $G_A$ can be viewed as a vector $x^A\in \set{0,1}^{\binom{V}{2}}$ and Bob's input graph $G_B$ can be viewed as a vector $x^B\in \set{0,1}^{\binom{V}{2}}$, where the coordinate $x^A_{(u,u)}$ indexed by the pair $u,u'$ of vertices in $V$ indicates whether or not the edge $(u, u')$ appears in graph $G_A$, and similarly $x^B_{(u,u')}$ indicates whether or not the edge $(u, u')$ appears graph $G_B$. It is then easy to see that the two players need to detect whether or not the bitwise-OR of vectors $x^A$ and $x^B$ is the all-one vector, which requires $\Omega(n^2)$-bits information exchange even in the back-and-forth communication model.
On the other hand, in the corresponding two-player one-way communication game for unweighted metric streams, Alice and Bob are each given a set of edge/non-edge information, with the promise that the edge/non-edge information between each pair of vertices appears in at least one of the player's input. There is a one-bit procoto: Alice simply sends to Bob a signal indicating whether or not in her input there is non-edge information between any pair of vertices, and Bob outputs ``Not a Clique'' iff either he sees Alice's "non-edge" signal or he sees a non-edge information in his input.


\iffalse
For example, consider the following star-identification problem: 
given an unweighted graph/metric stream, decide whether or not the underlying graph is a star graph that spans $n$ vertices.

On the one hand, there is a simple 2-pass $O(\log n)$ space algorithm for the star-identification problem in unweighted metric streams: in the first pass we store the first two edges that appear in the stream, if they do not share an endpoint, then return ``Not a Star''; otherwise record their common endpoint $u$, and then in the second pass only focus on whether or not there is any non-edge information $(u,v)$, and return that the graph is a star iff there is no such information. On the other hand, it is easy to show that, in unweighted graph streams, any $p$-pass algorithm has to use space $\Omega(n/p)$. Specifically, we can show that the corresponding two-player one-way communication game 
(in which Alice is given a subset $E_A\subseteq E(G)$ and Bob is given a subset $E_B\subseteq E(G)$, with the promise that $E_A\cup E_B=E(G)$, Alice is allowed to send a message to Bob, and Bob needs to return an answer upon receiving this message) 
has back-and-forth communication complexity $\Omega(n)$. In fact, consider the case that both Alice and Bob receives a subset of edges incident to a vertex $u$. Denote $V(G)=\set{u,v_1,\ldots,v_{n-1}}$, then this is equivalent to giving Alice a vector $x^A\in \set{0,1}^{n-1}$ and giving Bob a vector $x^B\in \set{0,1}^{n-1}$, where the $i$-th coordinate $x^A_i$ indicates whether or not the edge $(u, v_i)$ is in Alice's input edge set, and similarly the $i$-th coordinate $x^B_i$ indicates whether or not the edge $(u, v_i)$ is in Bob's input edge set. It is then easy to see that the two players need to detect whether or not the bitwise-OR of vectors $x^A$ and $x^B$ is the all-one vector, which requires $\Omega(n)$-bits information exchange even in the back-and-forth communication model.
\fi


The distinction that all non-edge information is explicitly given in the unweighted stream seems to fail all reductions from standard problems like Disjointness and Index) to prove lower bounds. Therefore, in the lower bound proofs of \Cref{thm: 1 pass alpha MST lower} and \Cref{thm: p pass alpha MST lower}, we identify new ``primitive'' graph-theoretic problems, prove communication lower bounds for them, and then reduce them to MST-estimation problems. Here we briefly provide some ideas for the proof of \Cref{thm: p pass alpha MST lower}.


We consider the special type of metrics, in which the distance between every pair of vertices is either $1$ or a large enough real number. Intuitively, the problem of estimating the MST weight is equivalent to the problem of estimating the number of connected component of the graph induced by all weight-$1$ edges, which is essentially a graph theoretic problem in unweighted metric streams.

As a first step, we consider the following problem: given an unweighted metric stream, decide whether the underlying graph is a perfect matching or a perfect matching minus one edge.
Unlike the previous star-identification problem, we show that corresponding two-player communication game for this problem has  communication complexity $\Omega(n)$ in the back and forth communication model, even if the complete edge/non-edge information is split between Alice and Bob. The proof is by analyzing the information complexity of any protocol for the problem,
We construct several similar input combinations for the Alice and Bob, among which some cross-combination lead to different answers, and then lower bound the mutual information between the procotol transcript and the players' inputs.

However, this perfect matching vs perfect matching minus one edge problem is not sufficient for our purpose, since a perfect matching graph on $n$ vertices has $n/2$ connected components, while a perfect matching minus one edge graph on $n$ vertices has $n/2-1$ connected components, and the ratio between $n/2$ and $n/2-1$ are too small to provide a space lower bound for $\alpha$-approximation of the number of connected components.
To fix this issue, we next consider a generalization of this problem, called the \emph{Clique or Independent Set} problem ($\coi_{a,b}$) parametrized by two integers $a,b$. In this problem, we are required to decide whether the input graph is the disjoint union of $b$ cliques of size $a$ each (Yes case) or it is a disjoint union of $(b-1)$ cliques of size $a$ each and an independent set of size $a$ (No case). Note that if $a=2$ and $b=n/2$ then this problem is exactly the perfect matching vs perfect matching minus one edge problem. Now if we let $a\gg b$, then the ratio between numbers of connected components in Yes case and in No case is $(a+b-1)/b=\Omega(a/b)$, which is enough for giving a space lower bound for $o(a/b)$-approximation streaming algorithms for MST estimation.
For the proof of the communication lower bound of problem $\coi_{a,b}$, we first consider the special case $\coi_{a,2}$ and show that the communication complexity is $\tilde\Omega(1)$ via a Hellinger distance analysis on transcript distributions on certain input combinations, and then use a direct sum type argument to show that the communication complexity of $\coi_{a,b}$ is $\tilde\Omega(b)$.
Both steps use techniques similar to the ones used in the proof of communication lower bound for the perfect matching vs perfect matching minus one edge problem.
Now for a given approximation ratio $\alpha>1$, setting $a=\Theta(\sqrt{\alpha n})$ and $b=\Theta(\sqrt{n/\alpha})$ yields the desired communication lower bound, which then implies the space lower bounds for streaming algorithms.



















==> special_metric.tex <==
\subsection{Optimality of \Cref{thm:coi}}


In this subsection, we show that the lower bound in \Cref{thm:coi} is asymptotically optimal in a mildly special case. In particular, if we additionally require that the input sets $\set{R_i}_{1\le i\le k}$ are disjoint, then the lower bound in \Cref{thm:coi} is almost tight.

%Specifically, we observe that the construction in the proof of \Cref{thm:coi} is quite special, and in this subsection we provide a streaming algorithm for MST estimation on this special class of metrics, achieving the space lower bound \Cref{thm: p pass alpha MST lower}. This result, conceptually, shows that the lower bound of \Cref{thm: p pass alpha MST lower} is almost tight in some sense.

Let $G$ be an unweighted graph. We define the \emph{$G$-complete stream} to be the sequence that contains a bit for every pair $v,v'$ of vertices of $V(G)$ indicating whether or not the edge $(v,v')$ belongs to $G$.
We say that a graph $G$ is \emph{nice}, iff $E(G)$ can be partitioned into disjoint sets, such that each set induces a clique on a subset of $V(G)$.
Consider the following streaming problem ${\sf ConCom}$: given a $G$-complete stream for some nice graph $G$, estimate the number of connected component of $G$.

In fact, \Cref{thm:coi} implies that any randomized $p$-pass $\alpha$-approximation streaming algorithm for the ${\sf ConCom}$ problem has to use $\Omega(\sqrt{n/\alpha p^2})$ space. In this subsection, we prove the following theorem, which shows that this lower bound is almost tight for ${\sf ConCom}$ problem.

\begin{theorem}
\label{Connected Component}
There is an $O(\log n)$-pass, $(1+\eps)$-approximation randomized algorithm for the ${\sf ConCom}$ problem, using $\tilde{O}(\sqrt{n})$ space. 
\end{theorem}

In particular, if we set $\alpha=O(1)$ and $p=O(\log n)$, then the lower bound in \Cref{thm:coi} tells us that such algorithm has to use at least $\tilde \Omega(\sqrt{n})$ space, and \Cref{Connected Component} shows that this bound is attainable.

%we consider a special case when the mectric only have two distances $1$ and $m$ where $m$ is larger than $2$. In this case, given three vertices $u$, $v$ and $w$ such that $d(u,v)=1$ and $d(v,w)=1$, we have $d(u,w)$ is also $1$. So each component in $G_1$ forms a clique. Denote $c$ as the number of cliques in $1$, the size of $\mst$ is $n-1+(c-1)(m-1)$. So in order to approximate the size of $\mst$, it is sufficient to approximate the value of $c$.

The remainder of this subsection is dedicated to the proof of \Cref{Connected Component}.

Let $c(G)$ be the number of connected component of the input graph $G$. We will construct two streaming algorithms $\alg_1$ and $\alg_2$, where $\alg_1$ will guarantee to return a $(1+\eps)$-approximation of $c(G)$ when $c(G)=\Omega(\sqrt{n})$, and $\alg_2$ will guarantee to return an $(1+\eps)$-approximation of $c(G)$ when $c(G)=\Omega(\sqrt{n})$. We then  run both algorithms in parallel through the stream and at the end decide to return the output of one of $\alg_1,\alg_2$. We now describe each of the algorithms in turn.
 
\paragraph{Algorithm $\alg_1$.}
We sample a subset $V'$ of $N=1000\sqrt{n}\log n/\eps^2$ vertices in $V$ uniformly at random at the start. For each vertex $v\in V'$, throughout the stream, we count the number of vertices that has distance $1$ from it, and denote this number by $X_v$. We then return $\hat c_1=(n/N)\cdot \sum_{v\in V'}(1/X_v)$. 
%Let $1/X_1,1/X_2,\dots, 1/X_N$ be the size of these cliques and $X$ be their sum.

We prove the following lemma.

\begin{lemma} \label{lem:1-m-app1}
If $c(G) \ge \sqrt{n}$, then with probability $1-O(n^{-100})$, $\card{\hat c_1-c(G)} < \eps \cdot c(G)$. 
\end{lemma}

\begin{proof}
Recall that graph $G$ is nice.
We denote by $\cset$ the set of all vertex-disjoint cliques whose union is $G$. Then 
$\sum_{v\in V} (1/X_v) = \sum_{C\in \cset} (|C|/|C|) = c(G)$. 
We let $X$ be the random variable that, for each $v\in V$, takes value $1/X_v$ with probability $1/n$.
Clearly, $X$ is supported on $[0,1]$ and $\expect[X]=c(G)/n$. On the other hand, $\hat c_1/n$ is the sample mean of $N$ samples of $X$.
%If we random sample a vertex $v$ and let $X_v=1/s_v$, then $\expect[X_v]=c/n$, which means $\expect[X \cdot n/N] = c$. On the other hand, since for each $v$, we have $1/s_v \in (0,1]$, 
From the Chernoff-Hoeffding inequality,
$$\Pr \bigg[\big|(\hat c_1/n)-\expect[X]\big| > \eps\cdot \expect[X] \bigg] \le  2\cdot \exp\bigg(-\frac{\eps^2\cdot N\cdot c(G)}{3}\bigg)=O(n^{-100}).$$
Therefore, with probability $1-O(n^{-100})$, $\card{\hat c_1-c(G)} < \eps \cdot c(G)$. 
\end{proof}

%By Lemma~\ref{lem:1-m-app1}, in the case of $c\ge \sqrt{n}$, we can approximate $c$ within a factor of $(1 \pm \eps)$ using $\tilde{O}(\sqrt{n})$ bits of space.

Before we describe the algorithm $\alg_2$, we need to first recall the notion of an $\ell_0$-sampler, a well-known tool in streaming algorithms. An $\ell_0$-sampler is a streaming algorithm, that, takes as input a real vector $a\in \mathbb{R}^n$ and a sequence of updates to the coordinates of $a$, and returns a uniformly at random non-zero coordinate of the resulting vector $a'$, namely a random element from $\set{i\mid a'_i\ne 0}$.

%\znote{from here}

\begin{proposition}[\!\!\!\cite{JowhariST2011}\!]\label{prop:ell-0-samplers}
There exists an $\ell_0$ sampler with zero relative error which uses $O(\log^2 n \log(1/\delta))$ space and outputs a coordinate $i \in [n]$ with probability at least $1 - \delta$ where $n$ is the size of the vector.
\end{proposition}


\paragraph{Algorithm $\alg_2$.}
%In the second algorithm, we will calculate $c$ accruately when $c$ is at most $\sqrt{n}$. To do so, we will use $\ell_0$ sampler algorithm. 
The second algorithm will run multi-pass. We first describe the first pass and the second pass. Before the first pass, we sample a set of $S$ with $1000\sqrt{n}\log n$ vertices. Let $V_S$ be the set of vertices that are in the same clique as some vertices in $S$ (note that we do not know the set $V_S$). During the first pass, if two vertices in $S$ has distance $1$ between them, then we delete arbitrary one from $S$. After the first pass, any two vertices in $S$ are not in the same clique, while $V_S$ does not change. In the second pass, we run $N=1000\sqrt{n}\log n$ $\ell_0$ samplers as follows: the vector has $n$ coordinates that represent the vertices, and set $\delta = n^{-100}$. Before the stream, we set the value on each coordinate as $1$ except the coordinates that represent vertices in $S$, they get value $0$. During the stream, if a vertex $v$ has distance $1$ from a vertex in $S$, we decrease the value on coordinate $v$ by $1$. In the end, all coordinates that represent vertices in $V_S$ has value $0$, and all other coordinates have value $1$. So by these $\ell_0$ samplers, we get $N$ samples from the set $V \setminus V_S$. We add these vertices into $S$. Then we run the third pass and forth pass in the same way as the first two passes, except that we are work on the new set $S$. We repeat this process until $V \setminus V_S = \emptyset$, then output $c=\card{S}$. Note that each two vertices in $S$ belongs to different cliques. So if $V_S=V$, then $c = \card{S}$, which means if the $\ell_0$ samplers never fail, we will get the correct answer.

\begin{lemma} \label{lem:1-m-app2}
    If $c \le \sqrt{n}$, the algorithm will stop in $2\log n$ passes with high probability.
\end{lemma}

\begin{proof}
    We first note that the failure probability of each $\ell_0$ sampler is $\delta=n^{-100}$, so with high probability, all $\ell_0$ samplers in the first $2\log n$ passes success. The following analysis is based on this event.

    We call each two passes a round, formly, each round starts right before we add the sampled vertices form $\ell_0$ samplers into $S$. We prove that the algorithm will terminate in $\log n$ rounds with high probability. To do so, we prove that in each round, the size of $V \setminus V_S$ will decrease by half with high probability.

    Suppose before some round, the size of $V \setminus V_S$ is $n'$. Since in the previous round, the $\ell_0$ samplers sample $N = 1000 \sqrt{n} \log n$ vertices in $V \setminus V_S$, for any cliques that at least $ n' /  2\sqrt{n}$, at least one vertex in the clique is sampled with probability $1- n^{-500}$. So after this round, with high probability, any clique with at least $2n' / \sqrt{n}$ vertices contains a vertex in $S$, which means for any vertex $v \in V \setminus V_S$, the clique that contains $v$ has size at most $n' /\sqrt{n}$. On the other hand, since $c \le \sqrt{n}$, we have $V \setminus V_S \le n'/2$.
\end{proof}

By Lemma~\ref{lem:1-m-app2}, the algorithm will stop in $\log n$ passes with high probability when $c \le \sqrt{n}$, and moreover, if the algorithm fails when $c \ge \sqrt{n}$, we know it fails. So can first run the second algorithm. If it terminates in $2 \log n$ passes, then we get a accurate $c$, otherwise we terminates it ourselves and run the first algorithm. The whole process uses $\tilde{O}(\sqrt{n})$ bits of space and take at most $2\log n + 1$ passes, and outputs an value $\hat{c}$ such that: if $c \le \sqrt{n}$, then $\hat{c}=c$, and $\card{\hat{c}-c} \le \eps c$ otherwise. So $(n-1)+(\hat{c}-1)(m-1)$ is a $(1 \pm \eps)$-approximation of $(n-1)+(\hat{c}-1)(m-1)$, which means we can get an approximation of the size of $\mst$ within a factor of $(1 \pm \eps)$.

